DPack: Efficiency-Oriented Privacy Budget Scheduling

Machine learning (ML) models can leak information about users, and differential privacy (DP) provides a rigorous way to bound that leakage under a given budget. This DP budget can be regarded as a new type of compute resource in workloads of multiple ML models training on user data. Once it is used, the DP budget is forever consumed. Therefore, it is crucial to allocate it most efficiently to train as many models as possible. This paper presents the scheduler for privacy that optimizes for efficiency. We formulate privacy scheduling as a new type of multidimensional knapsack problem, called privacy knapsack, which maximizes DP budget efficiency. We show that privacy knapsack is NP-hard, hence practical algorithms are necessarily approximate. We develop an approximation algorithm for privacy knapsack, DPack, and evaluate it on microbenchmarks and on a new, synthetic private-ML workload we developed from the Alibaba ML cluster trace. We show that DPack: (1) often approaches the efficiency-optimal schedule, (2) consistently schedules more tasks compared to a state-of-the-art privacy scheduling algorithm that focused on fairness (1.3-1.7x in Alibaba, 1.0-2.6x in microbenchmarks), but (3) sacrifices some level of fairness for efficiency. Therefore, using DPack, DP ML operators should be able to train more models on the same amount of user data while offering the same privacy guarantee to their users.

==> Makefile <==
PAPER=privacy_packing
LATEX=pdflatex

BIBTEX=bibtex

SRCS=$(PAPER).tex $(wildcard sections/*.tex)
REFS=$(wildcard bib/*.bib)
FIGS=$(wildcard figures/*)
STYLE=$(wildcard style/*)

.PHONY: results $(PAPER).pdf clean

all: results $(PAPER).pdf

results:
	+make -C $@

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS) $(STYLE)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)


submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

split: $(PAPER).pdf
	pdftk $(PAPER).pdf cat 1-14 output dpack_main.pdf
	pdftk $(PAPER).pdf cat 15 output dpack_appendix.pdf

clean:
	rm -f *.dvi *.aux *.log *.blg *.bbl \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps


==> results/Makefile <==
FIGS = placeholder/placeholder\
	motivating_examples_simulation/problem_1\
	motivating_examples_simulation/problem_2\
	single_block_killer/rdp_curves_block\
	single_block_killer/rdp_curves_normalized\
	single_block_killer/standard_epsilon_bound\
    single_block_killer/single_block_dpf_killer\
	multi_block_killer/rdp_curves\
    multi_block_killer/increasing_num_blocks/multi_block_dpf_killer\
	multi_block_killer/more_blocks_always_contention/multi_block_dpf_killer\
    single_block_killer_offline_schedulers/single_block_dpf_killer_offline_schedulers\
    multi_block_killer_offline_schedulers/multi_block_dpf_killer_offline_schedulers\
    offline_mixed_curves/offline_mixed_curves_without_profits\
	offline_mixed_curves/offline_mixed_curves_without_profits_runtime\
	online_batched_mixed_curves/delay_cdf_unlocked_T1\
	online_batched_mixed_curves/delay_cdf_locked_T1\
	online_batched_mixed_curves/online_batched_mixed_curves_N_without_profits_unlocked\
	online_batched_mixed_curves/delay_online_batched_mixed_curves_N_without_profits_unlocked\
	online_batched_mixed_curves/online_batched_mixed_curves_N_without_profits_locked\
	online_batched_mixed_curves/delay_online_batched_mixed_curves_N_without_profits_locked\
	privekube_workload/simulator/privekube_workload\
	privekube_workload/simulator/privekube_workload_profits_delay\
	privekube_workload/simulator/privekube_workload_no_profits\
	privekube_workload/simulator/privekube_workload_no_profits_delay\
	privekube_workload/simulator_sk/privekube_workload_profits_T\
	privekube_workload/simulator_sk/privekube_workload_profits_T_delay\
	privekube_workload/simulator_sk/privekube_workload_profits_ntasks\
	privekube_workload/simulator_sk/privekube_workload_profits_ntasks_delay\
	privekube_workload/simulator_sk/privekube_workload_noprofits_ntasks\
	privekube_workload/simulator_sk/privekube_workload_noprofits_ntasks_delay\
	privekube_workload/privekube/privekube_cdf_delay\
	privekube_workload/privekube/privekube_tasks_runtime_actual\
	rdp_curves_example/rdp_curves_example\
	rdp_curves_example/rdp_to_dp_curves_example\
	rdp_curves_example/rdp_curves_example_normalized\
	simplified_single_block_killer/subsampled\
	simplified_single_block_killer/gaussian\
	simplified_single_block_killer/normalized_rdp_curves_example\
	block_utilization/block_utilization\
	block_utilization/block_utilization_random\
	alibaba_workload/simulator/alibaba_max_blocks_100_lifetime_10\
	alibaba_workload/simulator/alibaba_max_blocks_100_lifetime_10_weights\
	heterogeneity_knobs/n_blocks_diversity\
	heterogeneity_knobs/best_alpha_diversity\
	alibaba_workload/simulator/alibaba_max_blocks_100_lifetime_10\
	alibaba_workload/simulator/alibaba_max_blocks_100_lifetime_10_weights\
	alibaba_workload/simulator/alibaba_max_blocks_100_lifetime_10_increasing_tasks\
	alibaba_workload/simulator/alibaba_max_blocks_100_lifetime_10_increasing_blocks\
	alibaba_workload/simulator/alibaba_increasing_blocks\
	alibaba_workload/simulator/alibaba_increasing_tasks\
	alibaba_workload/privekube/alibaba_tasks_runtime_actual\
	alibaba_workload/privekube/alibaba_cdf_delay\
	alibaba_workload/privekube/alibaba_increasing_tasks\
	alibaba_workload/simulator/alibaba_scheduling_delay\
	offline_heterogeneous_curves/heterogeneous_curves\
	offline_heterogeneous_curves/heterogeneous_curves_runtime\



GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal postscript eps enhanced monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES) $(PNGFILES)

